Determining interaction rules in animal swarms

In this paper we introduce a method for determining local interaction rules in animal swarms. The method is based on the assumption that the behavior of individuals in a swarm can be treated as a set of mechanistic rules. The principal idea behind the technique is to vary parameters that define a set of hypothetical interactions to minimize the deviation between the forces estimated from observed animal trajectories and the forces resulting from the assumed rule set. We demonstrate the method by reconstructing the interaction rules from the trajectories produced by a computer simulation.

==> figs/figure1a_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=129mm
% 
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{x}[][]{Hypothesis}
\psfrag{y}[][]{Force coefficient}
\psfrag{a}[][]{a}
\psfrag{b}[][]{b}
\psfrag{c}[][]{c}
\psfrag{d}[][]{d}
\psfrag{e}[][]{e}
\psfrag{f}[][]{f}
\psfrag{forcefactor}[][]{Parameter value}



==> figs/figure1b_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=129mm
% 
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{x}[][]{Hypothesis}
\psfrag{y}[][]{Force coefficient}
\psfrag{a}[][]{a}
\psfrag{b}[][]{b}
\psfrag{c}[][]{c}
\psfrag{d}[][]{d}
\psfrag{e}[][]{e}
\psfrag{f}[][]{f}
\psfrag{forcefactor}[][]{Parameter value}



==> figs/figure2a_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=129mm
% 
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{x}[][]{Hypothesis}
\psfrag{y}[][]{Force coefficient}
\psfrag{a}[][]{a}
\psfrag{b}[][]{b}
\psfrag{c}[][]{c}
\psfrag{d}[][]{d}
\psfrag{e}[][]{e}
\psfrag{f}[][]{f}
\psfrag{forcefactor}[][]{Parameter value}



==> figs/figure2b_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=129mm
% 
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{x}[][]{Hypothesis}
\psfrag{y}[][]{Force coefficient}
\psfrag{a}[][]{a}
\psfrag{b}[][]{b}
\psfrag{c}[][]{c}
\psfrag{d}[][]{d}
\psfrag{e}[][]{e}
\psfrag{f}[][]{f}
\psfrag{forcefactor}[][]{Parameter value}


